The Wisdom of Partisan Crowds: Comparing Collective Intelligence in Humans and LLM-based Agents

Human groups are able to converge on more accurate beliefs through deliberation, even in the presence of polarization and partisan bias -- a phenomenon known as the "wisdom of partisan crowds." Generated agents powered by Large Language Models (LLMs) are increasingly used to simulate human collective behavior, yet few benchmarks exist for evaluating their dynamics against the behavior of human groups. In this paper, we examine the extent to which the wisdom of partisan crowds emerges in groups of LLM-based agents that are prompted to role-play as partisan personas (e.g., Democrat or Republican). We find that they not only display human-like partisan biases, but also converge to more accurate beliefs through deliberation as humans do. We then identify several factors that interfere with convergence, including the use of chain-of-thought prompt and lack of details in personas. Conversely, fine-tuning on human data appears to enhance convergence. These findings show the potential and limitations of LLM-based agents as a model of human collective intelligence.

==> figures/agent_personas.tex <==
\begin{wrapfigure}[22]{R}{0.45\linewidth}
    % \begin{figure}[tbp!] 
    \centering
    \includegraphics[width=0.99\linewidth]{figures/agent_personas_fig.pdf}
    % \vspace{-4mm}
    \caption{Example detailed personas for a \textcolor{darkred}{Republican} agent (top) and a \textcolor{darkblue}{Democrat} agent (bottom) that an LLM agent role-plays.}
    \label{fig:agent_persona}
    \vspace{-4mm}
    % \end{figure}
\end{wrapfigure}


==> figures/aggregated_analysis_v2.tex <==
\begin{figure*}[htbp] % The * spans the figure across both columns
  \centering
  \includegraphics[width=0.9\linewidth]{figures/aggregate_analysis.pdf}
\end{figure*}

==> figures/becker_human_llm_eval.tex <==
\begin{figure*}[tbp!] 
\centering
\includegraphics[width=0.99\linewidth]{figures/becker_human_llm_eval_fig.pdf}
\vspace{-2mm}
\caption{\textbf{Top:} Average Normalized Group Error ($\overline{\varepsilon}$, and \textbf{Bottom:} Average Group Error Reduction ($\woc$) for (\textbf{A}) Human and (\textbf{B}) LLM Agents. The LLM agent result is from the condition with the highest alignment with human data, the condition with detailed persona and without CoT reasoning and induced partisanship. \sn{This figure needs to be replaced: remove the bar plot, and include the line plot across 6 prompt versions.}}
\label{fig:becker_human_vs_llm}
\vspace{-4mm}
\end{figure*}

==> figures/becker_human_vs_llm_plot.tex <==
\begin{figure*}[htbp] % The * spans the figure across both columns
  \centering
  \includegraphics[width=0.95\linewidth]{figures/becker_human_vs_llm_plot_fig_social_bias.pdf}
  \caption{The normalized group mean $\eta_{p,r,q}^t$ for each question for \textbf{(a)} The detailed result for each question for Role-Playing with detailed agent personas and without Chain-of-Thought reasoning. \textbf{(b)} The detailed result for each question for Fine-tuned Role-Playing with simple agent personas and without Chain-of-Thought reasoning. \textbf{(c)} The detailed results for each question for the human data. \sn{Should reshape it to 8 rows x 3 columns matrix.}}
  \label{fig:becker_human_vs_llm_plot}
\end{figure*}

==> figures/human_and_llm_left_panel.tex <==
\begin{figure}[thb!] 
    \centering

    \begin{subfigure}{\linewidth}
        \includegraphics[width=\linewidth]{figures/human_left_panel_fig.pdf}
        \caption{Human Data}
        \label{fig:human_left_panel}
    \end{subfigure}
    % Add some vertical space between the subfigures
    \vspace{1mm}
    \begin{subfigure}{\linewidth}
        \includegraphics[width=\linewidth]{figures/llm_v2_left_fig.pdf}
        \caption{LLM Agents Data}
        \label{fig:llm_v2_panel_left}
    \end{subfigure}

    % Optional overall caption and label
    \caption{Average Normalized Group Error ($\overline{\varepsilon_{social}^t}$ and $\overline{\varepsilon_{control}^t}$) for Social (solid line) and Control conditions (dotted line) across (a) human and (b) LLM agents. \sn{Should polish the figures. Should also include the detailed figure in the appendix.}}
    \label{fig:combined_figures_left}
    \vspace{-4mm}
\end{figure}

==> figures/human_and_llm_right_panel.tex <==
\begin{figure}[thbp!] 
    \centering

    \begin{subfigure}{\linewidth}
        \includegraphics[width=\linewidth]{figures/human_right_fig.pdf}
        \caption{Human Data}
        \label{fig:human_right_panel}
    \end{subfigure}
    % Add some vertical space between the subfigures
    \vspace{1mm}

    \begin{subfigure}{\linewidth}
        \includegraphics[width=\linewidth]{figures/llm_v2_right_fig.pdf}
        \caption{LLM Agents Data}
        \label{fig:llm_v2_panel_right}
    \end{subfigure}

    % Optional overall caption and label
    \caption{Average Group Error Reduction ($\overline{\Delta \varepsilon_{\text{social}}}$ and $\overline{\Delta \varepsilon_{\text{control}}}$) for Social and Control conditions across (a) human and (b) LLM agents. \sn{Should polush the figures}}
    \label{fig:combined_figures_right}
    \vspace{-4mm}
\end{figure}

==> figures/human_llm_v2_v4_fine_tuned_full_list_train.tex <==
\begin{figure*}[btp!] 
\centering
\includegraphics[width=0.65\linewidth]{figures/human_llm_v2_v4_fine_tuned_full_list_train_fig.pdf}
\vspace{-2mm}
\caption{}
\label{fig:becker_human_vs_llm_full_list_train}
\vspace{-4mm}
\end{figure*}

==> figures/human_vs_llm_across_prompt_versions.tex <==
\begin{figure*}[tbp!] 
\centering
\includegraphics[width=0.8\linewidth]{figures/human_vs_llm_across_prompt_versions_fig.pdf}
\vspace{-2mm}
\caption{Average Normalized Group Error ($\overline{\varepsilon}$) for (a) human crowds and (b) LLM agents across six experimental settings. Error bars indicating standard errors. \sn{Should include vicuna result as well.}\sn{Should use the term No CoT instead of Direct}}
\label{fig:becker_human_vs_llm}
\vspace{-4mm}
\end{figure*}

==> figures/human_vs_llm_across_prompt_versions_vertical_v1_to_v4.tex <==
\begin{figure}[bt!] 
\centering
\includegraphics[width=0.99\linewidth]{figures/human_vs_llm_across_prompt_versions_vertical_fig.pdf}
\vspace{-4mm}
\caption{Average Normalized Group Error ($\overline{\varepsilon}_t$) for (a) human crowds and (b) LLM agents (ChatGPT) across six experimental settings. Error bars indicating standard errors.}
% \sn{Consider having Vicuna result in the appendix.}
% \sn{Should think of a clever way to avoid the crowded legends.} 
\label{fig:becker_human_vs_llm}
\vspace{-4mm}
\end{figure}

==> figures/human_vs_llm_align_misalign.tex <==
\begin{figure*}[tbp!] 
\centering
\includegraphics[width=0.99\linewidth]{figures/human_vs_llm_align_misalign_fig.pdf}
\vspace{-2mm}
\caption{Human and LLM agent behavior in terms of the wisdom of crowds effect. The upper row shows a case where both (a) humans and (b) LLM agents demonstrate convergence towards the truth through social interaction (when estimating soldier causalities, $q=8$). In contrast, the lower row highlights a divergence where (c) humans show convergence towards the truth but (d) LLM agents do not (when estimating about the military budget, $q=5$). In each panel, the left subfigure shows the normalized group mean $\eta_{p,t}$ trajectory over three rounds, averaged across 12 group experiments (\textcolor{red}{red} for Republicans, \textcolor{blue}{blue} for Democrats), with error bars indicating standard errors. The right subfigure in each panel demonstrates the partial correlation $r_\text{adj}$ between the adjusted initial individual error $\widetilde{e}_{i,p,r,q}$ and adjusted estimate revisions $\widetilde{\Delta x}_{i,p,r,q}$ (both adjusted by the degree of social signals). A positive correlation indicates that those less accurate initially are more likely to revise their estimates. The results of the full set of questions are provided in \ref{app:result_revision_coefficient}.\sn{should define the per-question error reduction term.} \sn{Consider changing $r$ to $r_\text{adj}$  in the figure.} \sn{Should add an appendix for the complete set.}}
\label{fig:human_vs_llm_align_misalign}
\vspace{-4mm}
\end{figure*}


==> figures/llm_align_misalign_short_list.tex <==
\begin{figure*}[tbp!] 
\centering
\includegraphics[width=0.99\linewidth]{figures/llm_align_misalign_short_list_fig.pdf}
\vspace{-2mm}
\caption{Analysis of the mechanism of LLM agents' wisdom of crowds (WOC) effect at the individual level. Panel (a) shows the questions where LLM agents exhibit the WOC effect, characterized by the reduction in error ($\Delta \varepsilon < 0)$. Panel (b) shows the questions where LLM agents do not show the WOC effect. The left subfigures (line plots) illustrate the changes in normalized group mean $\eta_{p,t}$ over time for each question. The right subfigures (scatter plots) demonstrate the revision coefficient, the correlation $r_\text{adj}$ between the adjusted initial individual error $\widetilde{e}_{i,p,r,q}$ and adjusted estimate revisions $\widetilde{\Delta x}_{i,p,r,q}$ (\ref{sec:eval_metrics}). The LLM agents show the WOC effect only when $r_\text{adj}>0$. The results of the full set of questions are shown in Figure~\ref{fig:llm_align_misalign_full_list} (\ref{app:result_revision_coefficient}). \sn{Should add the complete figure to appendix.} \sn{Add stat test for the r value.}}
\label{fig:llm_align_misalign_short_list}
\vspace{-4mm}
\end{figure*}



==> figures/partisan_bias.tex <==
\begin{figure*}[tbp!] 
\centering
\includegraphics[width=0.99\linewidth]{figures/bias_combined_fig.pdf}
\vspace{-10mm}
\caption{To be added - nikunj}
\label{fig:partisan_bias}
\vspace{-4mm}
\end{figure*}

==> sections/ethic_statement.tex <==
\section*{Ethics Statement}

We will release the code base exclusively for research purposes.

\paragraph{U.S.-Centric Perspectives}
The authors, based in the U.S., acknowledge that their perspective, including references to minority groups, is shaped by this context and may not be globally applicable. The data that the study is based on \cite{becker2019wisdom} also recruited participants in the U.S.

\paragraph{Minority personas induced in LLMs models may not accurately represent real-world views}
We tried to induce minority personas in LLMs but we acknowledge that the LLMs have inherent biases due to the data that they have been trained on \cite{christiano2017deep, ziegler2019fine, feng2023pretraining}, and it is hard to steer these models to reflect personas of people belonging to minority demographics. Moreover, we also failed to recruit 'LLM agents' in a systematic way to include more diverse demographics.


==> sections/limitation.tex <==
\section*{Limitations}

\paragraph{Two-party political leaning}
Political orientation often extends beyond mere affiliation with two primary parties. In this research, we focused solely on personas identifying as either Democratic or Republican.

\paragraph{Non-exhaustive prompting strategies}
The current study only uses CoT prompting \cite{wei2022chain}, and doesn't explore other prompting strategies \citep{brown2020language, yao2023tree} due to limited time and budget. Previous work has shown the effect of prompting on model performance \citep{srivastava2022beyond, suresh2023conceptual}.  

% \paragraph{Fine-tuning only closed-source models} 
% Even thought we evaluate Vicuna-33B, an open-sourced model, in our experiment, we only fine-tuned ChatGPT and did not fine-tune Vicuna-33B.

\paragraph{Task limited to a number guessing game}
In this experiment, we employed a number guessing game to test the wisdom of crowds effect. This approach was chosen to emulate a similar task conducted previously by \cite{becker2019wisdom}, aiming to investigate how collective estimations or judgments made by a group can lead to accurate or insightful outcomes.



==> tables/result_fine_tune.tex <==
\begin{table*}[htb!]
    \centering
    % \small
    \resizebox{\linewidth}{!}{  
        \begin{tabular}{@{}llllllll@{}} 
            \toprule
            Method & $\overline{\Delta \varepsilon_{\text{s-c}}} \downarrow$ & $\overline{Bias_{\text{avg}}} \uparrow$ & $\overline{\Delta \varepsilon_{\text{social}}}$ & $\overline{Bias_{\text{social}}}$ & $\overline{\Delta \varepsilon_{\text{control}}}$ & $\overline{Bias_{\text{control}}}$ & $\ext$ \\ 
            \cmidrule(r{4pt}){1-3} \cmidrule(l{4pt}){4-8} % Adjusted line
            Raw Vanilla Role-playing & & & & & &\\
            \multicolumn{1}{@{\hspace{3em}}l}{Train set ($q \in [5,8]$)} & -10.46 & -10.67 & 7.51 & -20.76 & -2.95 & -0.57 & 0.00\\
            \multicolumn{1}{@{\hspace{3em}}l}{Test set ($q \in [1,4]$)} & 2.24 & 0.90 & 2.31 & 1.1 & 0.07 & 0.69 & 0.00 \\            
            \midrule
            Fine-tuned Vanilla Role-playing & & & & & &\\
            \multicolumn{1}{@{\hspace{3em}}l}{Train set ($q \in [5,8]$)} & -14.30 & -2.19 & -13.16 & 15.76 & 1.14 & 17.95 & 0.03\\
            \multicolumn{1}{@{\hspace{3em}}l}{Test set ($q \in [1,4]$)} & -10.95 & 0.63 & -13.83 & 1.00 & -2.88 & 0.37 & 25.84 \\            
            \midrule
            Human & & & & & & \\ 
            \multicolumn{1}{@{\hspace{3em}}l}{Train set ($q \in [5,8]$)} & -62.19 & 9.28 & -39.58 & 13.43 & 22.61 & 5.13 & 0.81 \\ 
            \multicolumn{1}{@{\hspace{3em}}l}{Test set ($q \in [1,4]$)} & -8.84 & 12.18 & -12.66 & 9.83 & -3.82 & 14.52 & 0.46 \\             
            \bottomrule
        \end{tabular}
    }
    \caption{Evaluation of fine-tuned LLM alignment with human group dynamics on the train set ($q \in [5,8]$) and the test set ($q \in [1,4]$). \sn{Should define the term "Raw Vanilla Rol-playing".}}
    \label{tab:result_fine_tune}
\end{table*}


==> tables/result_main.tex <==
\begin{table*}[htb!]
    \centering
    % \small
    \resizebox{\linewidth}{!}{  
        \begin{tabular}{@{}lllllllllll@{}}
            \toprule
            Model & Method & Persona & CoT & $\overline{\Delta \varepsilon_{\text{s-c}}} \downarrow$ & $\overline{Bias_{\text{avg}}} \uparrow$ & $\overline{\Delta \varepsilon_{\text{social}}}$ & $\overline{Bias_{\text{social}}}$ & $\overline{\Delta \varepsilon_{\text{control}}}$ & $\overline{Bias_{\text{control}}}$ & $\ext$ \\ 
            \cmidrule(r{4pt}){1-6} \cmidrule(l{4pt}){7-11}
            ChatGPT & Vanilla Role-playing & Detailed & CoT & 10.54 & 1.11 & -0.11 & 1.23 & -10.65 & 0.98 & 0.00 \\
             & & & \textbf{No CoT} & \textbf{-5.86} & \textbf{4.31} & -7.86 & 3.21 & -2.00 & 5.41 & 0.00 \\
             & & Simple & CoT & 13.79 & -11.97 & 0.83 & -15.91 & -12.96 & -8.02 & 0.00 \\
             & & & No CoT & -7.63 & -16.71 & -3.07 & -15.41 & 4.56 & -18.0 & 0.02 \\
             & Role-playing with Induced Partisanship & Simple & CoT & 8.89 & -1.88 &  2.63 & -0.01 & -6.26 & -3.75  & 0.00 \\
             & &  & No CoT & 1.52 & -15.58 & -1.01 & -24.22 & -2.53 & -6.92 & 0.00 \\
            \cmidrule(r{4pt}){2-6} \cmidrule(l{4pt}){7-11}
            Vicuna-33B & Vanilla Role-playing & Detailed & CoT & 4.99 & -0.42& 2.8 & 1.17 & -2.19 & -2.01 & 0.33 \\
             & & & \textbf{No CoT} & \textbf{-8.51} & \textbf{1.02} & -9.28 & 4.05 & -0.77 & -2.02 & 1.24 \\
             & & Simple & CoT & 6.03 & -1.29 & 3.21 & -0.85 & -2.82 & -1.73 & 0.25 \\
             & & & No CoT & -9.59 & -0.39 & -11.99 & 0.28 & -2.4 & -1.05 & 2.01 \\
             & Role-playing with Induced Partisanship & Simple & CoT &  32.71 & 21.8 & 42.35 & 28.09 & 9.64 & 15.51 & 3.63 \\
             & &  & No CoT & 3.77 & -3.22 & 1.35 & -3.24 & -2.42 & -3.2 & 1.39 \\
            \midrule
             Human & - & - & - & -35.51 & 10.73 & -26.12 & 11.63 & 9.39 & 9.82 & 0.64\\ 
            \bottomrule
        \end{tabular}
    }
    
    \caption{Evaluation of alignment between LLM agent and human group dynamics. The two main human-LLM alignment metrics are $\Delta \varepsilon_{\text{s-c}}$ (the more negative, the stronger the effect) and $\overline {Bias_{\text{avg}}}$ (the more positive, the more aligned with human). The highlighted row emphasizes the closest alignment of LLM role-playing with detailed personas to human group dynamics. \sn{Should define the term "Vanilla Role-playing" in the main text.} \sn{Should also include the standard errors in the table}}
    \label{tab:result_main}
\end{table*}


==> tables/result_vicuna.tex <==
% \begin{table*}[htb!]
%     \centering
%     % \small
%     \resizebox{\linewidth}{!}{  
%         \begin{tabular}{@{}llllllllll@{}}
%             \toprule
%             Method & Persona & CoT & $\overline{\Delta \varepsilon_{\text{s-c}}} \downarrow$ & $\overline{Bias_{\text{avg}}} \uparrow$ & $\overline{\Delta \varepsilon_{\text{social}}}$ & $\overline{Bias_{\text{social}}}$ & $\overline{\Delta \varepsilon_{\text{control}}}$ & $\overline{Bias_{\text{control}}}$ & $\ext$ \\ 
%             \cmidrule(r{4pt}){1-5} \cmidrule(l{4pt}){6-10} % Adjusted line
%             Vanilla Role-playing & Detailed & CoT & 4.99 & -0.42& 2.8 & 1.17 & -2.19 & -2.01 & 0.33 \\
%             & & \textbf{No CoT} & \textbf{-8.51} & \textbf{1.02} & -9.28 & 4.05 & -0.77 & -2.02 & 1.24 \\
%             & Simple & CoT & 6.03 & -1.29 & 3.21 & -0.85 & -2.82 & -1.73 & 0.25 \\
%             & & No CoT & -9.59 & -0.39 & -11.99 & 0.28 & -2.4 & -1.05 & 2.01 \\
%             Role-playing with Induced Partisanship & Simple & CoT &  &  &  &  &  &  &  \\
%             &  & No CoT & 3.77 & -3.22 & 1.35 & -3.24 & -2.42 & -3.2 & 1.39 \\
%             \midrule
%             Human & - & - & -35.51 & 10.73 & -26.12 & 11.63 & 9.39 & 9.82 & 0.64\\ 
%             \bottomrule
%         \end{tabular}
%     }
    
%     \caption{Evaluation of alignment between LLM agent and human group dynamics using vicuna-33b-v1.3. The two main human-LLM alignment metrics are $\Delta \varepsilon_{\text{s-c}}$ (the more negative, the stronger the effect) and $\overline {Bias_{\text{avg}}}$ (the more positive, the more aligned with human). The highlighted row emphasizes the closest alignment of LLM role-playing with detailed personas to human group dynamics.}
%     \label{tab:result_vicuna}
% \end{table*}


